VulDetectBench: Evaluating the Deep Capability of Vulnerability Detection with Large Language Models

Large Language Models (LLMs) have training corpora containing large amounts of program code, greatly improving the model's code comprehension and generation capabilities. However, sound comprehensive research on detecting program vulnerabilities, a more specific task related to code, and evaluating the performance of LLMs in this more specialized scenario is still lacking. To address common challenges in vulnerability analysis, our study introduces a new benchmark, VulDetectBench, specifically designed to assess the vulnerability detection capabilities of LLMs. The benchmark comprehensively evaluates LLM's ability to identify, classify, and locate vulnerabilities through five tasks of increasing difficulty. We evaluate the performance of 17 models (both open- and closed-source) and find that while existing models can achieve over 80% accuracy on tasks related to vulnerability identification and classification, they still fall short on specific, more detailed vulnerability analysis tasks, with less than 30% accuracy, making it difficult to provide valuable auxiliary information for professional vulnerability mining. Our benchmark effectively evaluates the capabilities of various LLMs at different levels in the specific task of vulnerability detection, providing a foundation for future research and improvements in this critical area of code security. VulDetectBench is publicly available at https://github.com/Sweetaroo/VulDetectBench.

==> data/exp/task45_specific.tex <==
\begin{table}[H]
    \centering
    \caption{Performance comparison of different models on Task 4 (Root Cause Location) and Task 5 (Trigger Point Location) for specific CWE types. The values represent the Unified Recall Score (URS) for each task, formatted as Task4|Task5. }
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lccccc}
            \toprule
            CWE for Model (TASK4|TASK5) & GPT4 & Gemini-pro & Deepseek & ChatGLM3 & QWEN(7B) \\
            \midrule
            CWE-78 OS Command Injection & 0.83|0.83 & 0.17|0.33 & 0.33|0.17 & 0.00|0.00 & 0.00|1.00 \\
            CWE-88 Argument Injection & 0.71|0.14 & 0.71|0.14 & 0.29|0.57 & 0.00|0.29 & 0.57|0.57 \\
            CWE-191 Integer Underflow & 0.00|0.14 & 0.00|0.57 & 0.00|0.57 & 0.00|0.14 & 0.29|0.86 \\
            CWE-89 SQL Injection & 0.83|0.00 & 0.33|0.33 & 0.00|0.33 & 0.00|0.17 & 0.00|0.50 \\
            CWE-476 NULL Pointer Dereference & 0.20|0.25 & 0.40|0.10 & 0.30|0.10 & 0.05|0.00 & 0.60|0.20 \\
            CWE-775 Missing Release of File Descriptor & 0.60|0.80 & 1.00|0.20 & 1.00|0.20 & 0.00|0.00 & 0.80|0.60 \\
            CWE-682 Incorrect Calculation & 0.00|0.00 & 0.25|0.50 & 0.25|0.00 & 0.00|0.00 & 0.00|0.25 \\
            CWE-120 Classic Buffer Overflow & 1.00|0.75 & 0.50|1.00 & 0.00|0.25 & 0.25|0.25 & 0.00|0.75 \\
            CWE-190 Integer Overflow or Wraparound & 0.00|0.00 & 0.33|0.00 & 0.00|0.33 & 0.00|0.00 & 0.00|0.68 \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:cwe_performance}
\end{table}

==> data/tables/finetune.tex <==
% \begin{table}[htb]
% 	\centering
% 	\caption{Finetune results comparison.}
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{lcccc}
% 			\toprule
% 			Model  &  Size  &    \makecell{Task 3   \\ MAR|   MIR }&  \makecell{Task 4  \\  URS  | ORS  } & \makecell{Task 5  \\ URS | ORS   } \\
% 			\midrule
% Llama3 & 8B  & 22.83 |   17.99 & 00.19 |   01.10           & 00.17 |   00.53  \\
% Llama3(fine-tuned) & 8B  & 27.98 |   25.56 & 91.80 |   92.89          & 90.19 |   90.61\\
% 			\bottomrule
% 		\end{tabular}
% 		\label{tab:finetune-results}
% 	}
	
% \end{table}

\begin{table}[ht]
	\centering
        \small
	\caption{Overall Results. For each of the five tasks in the VulDetectBench, we evaluate 17 LLMs, three of which were closed-source models, using two metrics. The specific types of these models are described in detail in the Appendix.}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{lcccc}
			\toprule
			Model  &  Size  &   \makecell{Task 3   \\ MAR|   MIR }&  \makecell{Task 4  \\  URS  | ORS  } & \makecell{Task 5  \\ URS | ORS   } \\
			\midrule
			GPT4 & -    &   20.21 |   16.07 &  24.26 |   27.07 & 13.00 |   17.85 \\
			ERNIE4.0    & -    &  27.87 |   22.54 & 11.77 |   27.99 & 22.43 |   10.38 \\
			Gemini-pro  & -                      &   13.03 |   10.55 & 14.64 |   23.51          & 07.56 |   18.89          \\
			Deepseek & 7B &    17.81 |   13.67 & 05.36 |   09.22          & 04.30 |   08.83          \\
			Qwen & 7B                                         & 13.63 |   11.15 & 04.34 |   10.09          & 05.56 |   10.95          \\
			Qwen & 14B                                       & 16.49 |   13.67 & 06.40 |   08.32          & 03.14 |   04.81          \\
			ChatGLM3 & 6B                                             & 00.16 |   00.12 & 00.19 |   01.33          & 00.42 |   01.12          \\
			Vicuna & 13B                                        & 07.30 |   06.35 & 0 |   0                 & 0 |   0                \\
			Vicuna & 7B                                        & 07.79 |   06.24 &  0 |   0                & 0 |   0                \\
			CodeLlama & 13B                            & 10.34 |   08.51 & 03.30 |   03.47          & 01.29 |   01.89          \\
			CodeLlama & 7B                                 & 06.28 |   05.04& 01.69 |   02.55          & 00.69 |   01.31          \\
			
			Llama3 & 8B                                 & 22.83 |   17.99 & 00.19 |   01.10           & 00.17 |   00.53          \\
			Llama2 & 7B                                       & 11.47 |   09.59 & 0 |   0                 & 0 |   0                \\
			Llama2 & 13B                                    & 10.99 |   09.23 & 00.50 |   01.20           & 00.10 |   00.20          \\
			Llama3 & 70B                                             & 09.18 |   07.43 & 0 |   0                 & 0 |   0                 \\
			Mixtral & 8*7B                                           & 21.61 |   17.51 & 01.66 |   04.28          & 05.74 |   03.51          \\
			Mixtral & 8 *22B                                      &  \textbf{30.26  |   24.10} & 17.49 |   11.46          & 06.17 |   02.83     \\    
            \textbf{Llama3(fine-tuned)} & 8B  & \textbf{27.98 | 25.56} & \textbf{91.80 | 92.89}     &\textbf{ 90.19 | 90.61}\\
			\bottomrule
		\end{tabular}
		\label{tab:fintune_result}
	}
	
\end{table}

==> data/tables/hundred.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}
% 	\caption{Horizontal Comparison}
% 	\label{tab:hundred}
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{lccccc}
% 			\toprule
% 			& TASK1& TASK 2 & TASK3 & TASK4 & TASK5 \\
% 			\midrule
% 			GPT4   & 1.00    & 0.765|0.860  & 0.2021|0.1607  & 0.2426|0.2707  & 0.1300|0.1785                                                   \\
% 			Gemini-Pro   & 0.58  & 0.510|0.590  & 0.1303|0.1055  & 0.1464|0.2351  & 0.0756|0.1889    \\
% 			Qwen1.5-14B  & 0.60   & 0.575|0.660   & 0.1649|0.1367  & 0.0640|0.0832   & 0.0314|0.0481                                                   \\
% 			Meta-Llama-8B   & 1.00    & 0.525|0.620    & 0.2283|0.1799    & 0.0017|0.0053  & 0.0019|0.0110                                                   \\
% 			Deepseek-coder-7b & 0.70   & 0.160|0.200   & 0.1781|0.1367  & 0.0536|0.0922    & 0.0430|0.0883     \\                        
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% \end{table}
